Counterfactually Measuring and Eliminating Social Bias in Vision-Language Pre-training Models

Vision-Language Pre-training (VLP) models have achieved state-of-the-art performance in numerous cross-modal tasks. Since they are optimized to capture the statistical properties of intra- and inter-modality, there remains risk to learn social biases presented in the data as well. In this work, we (1) introduce a counterfactual-based bias measurement \emph{CounterBias} to quantify the social bias in VLP models by comparing the [MASK]ed prediction probabilities of factual and counterfactual samples; (2) construct a novel VL-Bias dataset including 24K image-text pairs for measuring gender bias in VLP models, from which we observed that significant gender bias is prevalent in VLP models; and (3) propose a VLP debiasing method \emph{FairVLP} to minimize the difference in the [MASK]ed prediction probabilities between factual and counterfactual image-text pairs for VLP debiasing. Although CounterBias and FairVLP focus on social bias, they are generalizable to serve as tools and provide new insights to probe and regularize more knowledge in VLP models.

==> tables/retrieval_zeroshot.tex <==
\begin{table}[t]

  \setlength{\abovecaptionskip}{1pt}
%   \setlength{\belowcaptionskip}{-0.5cm}
  \caption{Zero-shot image-text retrieval results on Flickr30K.}
  	\label{downzero}
  
%     \small
% 	\centering	
%     \aboverulesep = 0.46mm
%     \belowrulesep = 0.46mm
% \setlength\tabcolsep{5pt}
% 	\resizebox{0.75\textwidth}{!}
{
	\begin{tabular}	{l   |  c  c  c  c  c  c  }
		\toprule	 	
	 \multirow{2}{*}{Method} & \multicolumn{6}{c}{Flickr30K (1K test set)}\\
	  &  \multicolumn{3}{c}{TR}& \multicolumn{3}{c}{IR} \\
	 \midrule
	&  R@1 &R@5&R@10& R@1 &R@5&R@10 \\
	%ImageBERT~\cite{ImageBERT} & 2M &70.7 & 90.2 & 94.0 & 54.3 & 79.6 & 87.5 \\
	Vanilla  & 83.6 & 95.7 & 97.7 & 68.7 & 89.2 & 93.9 \\
	FairVLP  & 88.0 & 98.7 & 99.4 & 68.7 & 90.6 & 95.2 \\

		\bottomrule
	\end{tabular}
%  	}
%  	 \vspace{-0.8ex}
% 	\caption
% 	{
% % 	\small	
% 		
% 	}
}
    % \vspace{-0.7ex}
\end{table}		
